SciInstruct: a Self-Reflective Instruction Annotated Dataset for Training Scientific Language Models

Large Language Models (LLMs) have shown promise in assisting scientific discovery. However, such applications are currently limited by LLMs' deficiencies in understanding intricate scientific concepts, deriving symbolic equations, and solving advanced numerical calculations. To bridge these gaps, we introduce SciInstruct, a suite of scientific instructions for training scientific language models capable of college-level scientific reasoning. Central to our approach is a novel self-reflective instruction annotation framework to address the data scarcity challenge in the science domain. This framework leverages existing LLMs to generate step-by-step reasoning for unlabelled scientific questions, followed by a process of self-reflective critic-and-revise. Applying this framework, we curated a diverse and high-quality dataset encompassing physics, chemistry, math, and formal proofs. We analyze the curated SciInstruct from multiple interesting perspectives (e.g., domain, scale, source, question type, answer length, etc.). To verify the effectiveness of SciInstruct, we fine-tuned different language models with SciInstruct, i.e., ChatGLM3 (6B and 32B), Llama3-8B-Instruct, and Mistral-7B: MetaMath, enhancing their scientific and mathematical reasoning capabilities, without sacrificing the language understanding capabilities of the base model. We release all codes and SciInstruct at https://github.com/THUDM/SciGLM.

==> examples/output_scieval.tex <==
\begin{figure*}[h!]
\fbox{\begin{minipage}{0.98\textwidth}
\scriptsize
\textbf{Problem} How does electric field affect capacitance?\\\\
A. Electric field decreases capacitance.\\
B. Electric field doesn't affect capacitance.\\
C. Electric field changes capacitance based on geometry.\\
D. Electric field increases capacitance.
% \textbf{category:} physics;
% \textbf{topic:} Electric Forces and Fields;
% \textbf{ability:} Scientific Calculation;
% \textbf{type:} multiple-choice;
% \textbf{task\_name:} SocraticQA.
\end{minipage}}
\fbox{\begin{minipage}{0.98\textwidth}
\scriptsize
\textbf{Correct Answer}\\
B       
\end{minipage}}
\fbox{\begin{minipage}{0.98\textwidth}
\scriptsize
\textbf{Answer produced by ChatGLM3-6B-Base}\\
\xmarkcolor \quad D        
\end{minipage}}
\fbox{\begin{minipage}{0.98\textwidth}
\scriptsize
\textbf{Answer produced by \model (ChatGLM3-6B-Base)}\\
\checkmarkcolor \quad B 
\end{minipage}}
\vspace{-1mm}
\caption{An example problem from SciEval is accurately solved by \model (ChaGLM3-6B-Base). For this problem, the category is physics; the topic is Electric Forces and Fields; the ability is Scientific Calculation; the type is multiple-choice; the task name is SocraticQA.}
\label{appendix:output_example}
\end{figure*}

==> mdframed/GPT-4_Labeling.tex <==
% \afterpage{
\begin{mdframed} %[tikzsetting={draw=none}]
\centering
\label{GPT-4 Labeling}
\textbf{GPT-4 Labeling} 
\begin{mdframed}
\textbf{Prompt: } 
The following input includes three segments. It starts with a question, followed by a step-by-step solution to the question, and ends with the true answer. If the answer obtained in the solution is equivalent to the real one, output ‘1’, otherwise output ‘0’.
\end{mdframed}

\begin{mdframed}
\textbf{Input }

\textbf{Q: }{A photon moving at speed c, a person chasing light at 0.9c, that person observes the speed of light is?}

\textbf{Solution: }{According to Einstein's theory of special relativity, we cannot simply add up the velocities. In relativity, the superposition of velocities follows the Lorentz transformation, rather than the classical addition. For the speed of light, there is a special case in which the observer measures the speed of light as c, regardless of the observer's speed. This means that even if an observer is moving at 0.9c, the speed of light he measures is still c. Therefore, the speed of light observed by this person is c.}

\textbf{Real Answer: }{c.}
\end{mdframed}

\begin{mdframed}
\textbf{GPT-4 Output:}{ 1}
\end{mdframed}

\end{mdframed}
% }

==> mdframed/Solution_with_CoT_Prompting_on_Physics.tex <==

\afterpage{
\begin{mdframed}
\label{cot_sample_physics}
\textbf{Solution with CoT Prompting on Physics} \\
\textbf{Problem: } 
A particle for simple harmonic vibration, the period is T. When it moves from the equilibrium position to the positive direction of the x-axis, from the equilibrium position to the maximum displacement of half the time required is $\\A, T/12.\\ B, T/8.\\ C, T/6. \\D, T/4$.

\textbf{Analysis: }
The displacement of a harmonic vibration can be expressed as:
\[x = A\cos(\omega t + \phi)\]

where:
\(A\) is the amplitude,
\(\omega\) is the angular frequency,
\(\phi\) is the initial phase, and
\(t\) is the time.

The period \(T\) is given by \(T = \frac{2\pi}{\omega}\), so \(\omega = \frac{2\pi}{T}\). 

To find the time it takes to reach half of the maximum displacement (\(\frac{1}{2}A\)), we set \(x = \frac{1}{2}A\). Since the equilibrium position is the central position of the vibration, the initial phase \(\phi = 0\) or \(\phi = \pi\). 
Also, since the motion is in the positive X-axis, \(\phi = 0\). 

Plugging in \(x = \frac{1}{2}A\), we get:
\[\frac{1}{2}A = A\cos(\omega t)\]

Simplifying further:
\[\cos(\omega t) = \frac{1}{2}\]

This implies:
\[\omega t = \frac{2t\pi}{T} = \frac{\pi}{3} \text{ or } \frac{5\pi}{3}\]

So, \(t = \frac{T}{6}\) or \(\frac{5T}{6}\). Since the motion starts from the equilibrium position, the correct answer is \(t = \frac{T}{6}\). Therefore, the correct answer is \(C,  \frac{T}{6}\).

\textbf{Final Answer:} Therefore, the correct answer is \(C, \frac{T}{6}\). 

\textbf{Real Answer:} C
\end{mdframed}
}


==> tables/data_source.tex <==
\begin{table*}[!th]
    \centering
    \caption{An overview of the main sources used for each subject area.}
    % \resizebox{110mm}{!}{
    \begin{tabular}{l|l|l}
    \hline
        Subject & Source & Description \\ 
    \hline
    Lean &
        \url{https://zenodo.org/records/10114157} & open-source \\ 
    \hline
         \multirow{10}{*}{Physics}& college physics series textbook 1 \footnote{https://lib-tsinghua.wqxuetang.com/book/3207349}
         & Obtained permission from publisher \\ 
         & college physics series textbook 2 
         \footnote{https://lib-tsinghua.wqxuetang.com/book/3207181} & Obtained permission from publisher \\ 
         & college physics series textbook 3 \footnote{https://reserves.lib.tsinghua.edu.cn/Search/BookDetail?bookId=11ad92b1-d4f1-4ea9-8d2c-310640ba96b1} & Obtained permission from publisher \\ 
         & physics dictionary series textbook 1 \footnote{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=BEB02D0B8BB9A43A8B97D3B4B193BDD0C000} & Obtained permission from publisher \\ 
         & physics dictionary series textbook 2 \footnote{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=BFE5E7D8A9D834A89A1D6EE617F4B56EE000} & Obtained permission from publisher \\ 
         & physics dictionary series textbook 3 \footnote{https://reserves.lib.tsinghua.edu.cn/Search/BookDetail?bookId=adf6ebfd-f306-4cfc-a9e1-1a95d5c5cc01} & Obtained permission from publisher \\ 
         & physics dictionary series textbook 4 \footnote{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=BAFF531EE50E3445CBA17C5A743ED0725000} & Obtained permission from publisher \\ 
         & physics dictionary series textbook 5 \footnote{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=B754358F367D3135BE053020B0A0AB3A6000} & Obtained permission from publisher \\ 
         & physics dictionary series textbook 6 \footnote{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=BD69B279D75CB4703A387EF03E9E8B094000} & Obtained permission from publisher \\ 
         & physics dictionary series textbook 7 \footnote{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=B091D287D415D4C9DAD1F500E60AE6F0F000} & Obtained permission from publisher \\ 
    \hline
        Chemistry & pedagogical materials & Obtained permission from teacher \\ 
    \hline
        Math & \url{https://www.bartleby.com/} & open-access, Q\&A written by humans \\ 
    \hline
    \end{tabular}
    % }
    \begin{tablenotes}    
        \scriptsize              
        \item[1] [1] \url{https://lib-tsinghua.wqxuetang.com/book/3207349}

        \item[2] [2] \url{https://lib-tsinghua.wqxuetang.com/book/3207181}
        
        \item[3] [3] \url{https://reserves.lib.tsinghua.edu.cn/Search/BookDetail?bookId=11ad92b1-d4f1-4ea9-8d2c-310640ba96b1}
        
        \item[4] [4] \url{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=BEB02D0B8BB9A43A8B97D3B4B193BDD0C000}
        
        \item[5] [5] \url{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=BFE5E7D8A9D834A89A1D6EE617F4B56EE000}
        
        \item[6] [6] \url{https://reserves.lib.tsinghua.edu.cn/Search/BookDetail?bookId=adf6ebfd-f306-4cfc-a9e1-1a95d5c5cc01}
        
        \item[7] [7] \url{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=BAFF531EE50E3445CBA17C5A743ED0725000}
        
        \item[8] [8] \url{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=B754358F367D3135BE053020B0A0AB3A6000}
        
        \item[9] [9] \url{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=BD69B279D75CB4703A387EF03E9E8B094000}
        
        \item[10] [10] \url{https://book.sciencereading.cn/shop/book/Booksimple/show.do?id=B091D287D415D4C9DAD1F500E60AE6F0F000}
    \end{tablenotes}   
    \label{tab:data_source}
\end{table*}




==> tables/general_results.tex <==
\begin{table}[t!]
    \centering
    \caption{\textbf{Results on general language understanding tasks}. Fine-tuning does not sacrifice most language tasks and only drops a bit on the code generation task. 
    }
    \begin{threeparttable} 
    \resizebox{!}{15mm}{
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}ccccc@{}}
    % \begin{tabular}{c|c|c|c|c|c|c|c}
    \specialrule{.10em}{.4ex}{.65ex}
         Model & MMLU & CEval & MBPP &Avg.\\
         \specialrule{.10em}{.4ex}{.65ex}
         GPT-4 & 86.40  &68.70 &83.00 &79.37  \\
         \specialrule{.10em}{.4ex}{.65ex}
         ChatGLM3-6B-Base  & 61.32	&67.09	&55.80  &61.40 \\
         \textbf{\model} (6B-Base) &61.38	&67.16	&45.00	&57.85 \\
         \specialrule{.10em}{.4ex}{.65ex}
         ChatGLM3-32B-Base &69.05	&{79.94}	 &{58.20}   &69.06 \\
         \textbf{\model} (32B-Base)  &{70.08} &79.64 &56.60  &68.78\\
         \specialrule{.16em}{.4ex}{0pt}
    \end{tabular}
    }
    \end{threeparttable}
    \label{tab:general_results}
\end{table}

==> tables/subject_results.tex <==
\begin{table}[t]
    \centering
    \caption{Impact of the subject, w.r.t., average benchmarks.}
    % \setlength{\tabcolsep}{1.5mm}{
    % \begin{tabular}{c|c|c|c}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}cccc@{}}
        \specialrule{.10em}{.4ex}{.65ex}
         Subject Setting & Ave. Math & Ave. Sci & Ave. Bench  \\
                  \specialrule{.10em}{.4ex}{.65ex}
         w/o Math &39.06 &51.81 &44.16 \\
                  \specialrule{.10em}{.4ex}{.65ex}
         w/o Theorem Proof &\underline{40.57} &\underline{53.38} &\underline{45.69} \\
                  \specialrule{.10em}{.4ex}{.65ex}
         w/o Physics \& Chemistry &39.46 &49.84 &43.61 \\
         \specialrule{.10em}{.4ex}{.65ex}
         \model &\textbf{42.40} &\textbf{54.28} &\textbf{46.36} \\
                  \specialrule{.16em}{.4ex}{0pt}
    \end{tabular}
    }
    \label{tab:ablation}
\end{table}
